Diffusion Self-Guidance for Controllable Image Generation

Large-scale generative models are capable of producing high-quality images from detailed text descriptions. However, many aspects of an image are difficult or impossible to convey through text. We introduce self-guidance, a method that provides greater control over generated images by guiding the internal representations of diffusion models. We demonstrate that properties such as the shape, location, and appearance of objects can be extracted from these representations and used to steer sampling. Self-guidance works similarly to classifier guidance, but uses signals present in the pretrained model itself, requiring no additional models or training. We show how a simple set of properties can be composed to perform challenging image manipulations, such as modifying the position or size of objects, merging the appearance of objects in one image with the layout of another, composing objects from many images into one, and more. We also show that self-guidance can be used to edit real images. For results and an interactive demo, see our project page at https://dave.ml/selfguidance/

==> suppmattext.tex <==
\renewcommand*{\thesubsection}{\Alph{subsection}.}
\setcounter{subsection}{0}

\makeatletter
\newcommand{\iflabelexists}[3]{\@ifundefined{r@#1}{#3}{#2}}
\makeatother

\newcommand{\reff}[2]{\iflabelexists{#1}{\ref{#1}}{#2}}

\subsection{Implementation details}
We only apply our self-guidance term at sampling steps where classifier-free guidance is also applied. In our model, the default classifier-free guidance schedule is defined as the following: for a sampling process with $N$ DDPM steps, the first $\frac{3N}{16}$ steps use guidance (both classifier-free and self-guidance), the last $\frac{N}{32}$ use no guidance, and the remaining middle $\frac{25N}{32}$ steps alternate between guidance and no guidance. For results shown in the paper, we use $N=1024$ DDPM steps, but have found our method works with $256$ and $512$ steps as well, though self-guidance weights may require adjustment. We set $v=7500$ in Eqn.~\reff{eq:propmatch}{5} in the paper as an overall scalar for the gradients of the functions $g$ defined below. We find that the magnitude of per-pixel gradients produced by the terms we consider is quite small (often in the range of $10^{-7}$ to $10^{-6}$), so a high weight is needed to induce changes.

We apply \texttt{centroid}, \texttt{size}, and \texttt{shape} terms on {\em all} cross-attention interactions. In our model, there are a total of 36 of these at varying resolutions: $8\times 8$, $16\times 16$, and $32\times 32$. We apply the \texttt{appearance} term using the activations of the penultimate layer in the decoder (that is, two layers before the prediction readout) as well as the final cross-attention operation. Both tensors are $32 \times 32$.

When using our cascaded upsampling models that go from $64\rightarrow256$px and $256\rightarrow1024$px, we keep all sources of randomness fixed across original and generated images to preserve maximal consistency.

\paragraph{Attention mask binarization.}
In practice, it is beneficial to differentiably binarize the attention map (with sharpness controlled by $s$) before computing its size or utilizing its shape, to eliminate the effect of background noise (this is empirically less important when guiding centroids, so we do not binarize in that case). We take a soft threshold at the midpoint of the per-channel minimum and maximum values. More specifically, we apply a shifted sigmoid on the attention normalized to have minimum 0 and maximum 1, followed by another such normalization to ensure the high value is 1 and the low value is 0 after applying the sigmoid. We use $s=10$ and redefine Eqn.~\reff{eqn:size}{10} from the main paper as:
\begin{gather}
    \texttt{normalize}(\mathbf{X}) = \frac{\mathbf{X} - \min_{h,w}\left(\mathbf{X}\right)}{\max_{h,w}\left(\mathbf{X}\right) - \min_{h,w}\left(\mathbf{X}\right)} \\
    \attn^\text{thresh} = \texttt{normalize}\left(\texttt{sigmoid} \left(s \cdot \left(\texttt{normalize}(\attn) - 0.5 \right)\right)\right) \\
    \texttt{size}\left(o\right) = \frac{1}{HW}\sum_{y,x} \attnsingle^\text{thresh} %
\end{gather}

\subsection{Using self-guidance}
\paragraph{Maximizing consistency.} In general, we find that sharing the same sequence of noise in the DDPM process between an image and its edited version is {\em not necessary} to maintain high levels of consistency, but can help if one desires to preserve very fine details between the original and edited image. We also find that object silhouettes are better preserved after spatial transformations such as resizing and repositioning when applying guidance towards the original $\texttt{shape}$ under a transformation $\mathcal{T}$, rather than expressing the same change through $\texttt{centroid}$ and $\texttt{size}$.

\paragraph{Guiding ``background'' words.} To keep all but one object fixed (a common use-case, shown in Fig.~\reff{fig:spatial_single_object}{3}), one can either guide all other tokens in the prompt (including ``a photo of'' and other abstract terms) to maintain their original properties, or only select the other salient objects and hold those fixed. In general, since abstract words are often used as message-passing conduits and have attention patterns that are meaningfully correlated with the layout of the scene (in particular the background, whose visibility betrays the location of foreground objects), we generally prefer not to guide their layouts to maximize compositionality of terms across images. However, guiding them can help keep specific details of the scene fixed in certain cases.
\begin{figure}
    \input{figures/supp/moveobjs}
    \caption{\textbf{Moving objects.} Random, non-cherry-picked results for moving objects in scenes using Eqn.~\ref{eqn:moveobj}. We move \texttt{onion} diagonally down and to the right, \texttt{pineapple} to the right, and \texttt{owl} up and \texttt{pig} down, respectively. All scenes use weights $w_0=1.5$, $w_1=0.25$, and $w_2=2$. }
    \label{fig:moveobjsupp}
    \vspace{-0.5em}
\end{figure}

\paragraph{Pooling across tokens.} When words or concepts span multiple tokens, we have the choice of mean-pooling their attention maps across these tokens before proceeding with them. We do not find this to make a noticeable difference, so choose not to mean-pool before processing for simplicity, but in some cases doing so may be desirable ({\em e.g.} to minimize the appearance leakage of a layout guidance term). 

We take the mean spatially of all \texttt{shape} terms and across activation dimensions for all \texttt{appearance} terms, which we omit below for conciseness.

\paragraph{Moving objects.} 
For a given caption $C$ with words at indices $\{c_i\}$, in which $N=\{n_j\} \subseteq C$ are nouns, we can move an object $n_k$ at timestep $t$ (with noised image $z_t$) with:
\begin{equation}
\begin{aligned}
    g &= w_0 \overbrace{ \frac{1}{|C|-1} \sum_{c \neq n_k \in C}\frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|}   \| \texttt{shape}_{i,t,\text{orig}}(c) - \texttt{shape}_{i,t}(c) \|_1 }^\text{Fix all other token shapes} \\
    &+ w_1 \overbrace{  \frac{1}{|C|} \sum_{c \in C} \| \texttt{appearance}_{t,\text{orig}}(c) - \texttt{appearance}_{t}(c) \|_1 }^\text{Fix all appearances} \\
    &+ w_2 \underbrace{ \frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|} \| \mathcal{T}\left(\texttt{shape}_{i,t,\text{orig}}(n_k)\right) - \texttt{shape}_{i,t}(n_k) \|_1 }_\text{Guide $n_k$'s shape to translated original shape}
\end{aligned}
\label{eqn:moveobj}
\end{equation}
Where $\texttt{shape}_\text{orig}$ and $\texttt{shape}$ are extracted from the generation of the initial and edited image, respectively. Critically, $\mathcal{T}$ lets us define whatever transformation of the $H_i\times W_i$ spatial attention map we want. To move an object, $\mathcal{T}$ translates the attention mask the desired amount (using bilinear interpolation to sample). We generally use weights $w_0 \in [0.5, 2], w_1 \in [0.03,0.3], w_2 \in [0.5, 5]$.

\begin{figure}
    \input{figures/supp/resizeobjs}
    \caption{\textbf{Resizing objects.} Random, non-cherry-picked results for resizing objects in scenes using Eqn.~\ref{eqn:moveobj}, with $\mathcal{T}$ specified to up- or down-sample the attention maps of interest. We shrink the \texttt{punching bag} $0.5\times$ along the $y$ axis, enlarge the chicken $2.5\times$, and enlarge the boombox $2\times$. All scenes use weights $w_0=2$, $w_1=0.25$, and $w_2=3$. }
    \label{fig:resizeobjsupp}
    \vspace{-1.5em}
\end{figure}

Alternatively, we can keep the first terms from the above equation, and express $n_k$'s new location through the \texttt{centroid} operation, adding a term to keep its \texttt{size} fixed:
\begin{equation}
\begin{aligned}
    g &= w_0 \overbrace{  \frac{1}{|C|-1}\sum_{c \neq n_k}\frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|}     \| \texttt{shape}_{i,t,\text{orig}}(c) - \texttt{shape}_{i,t}(c) \|_1 }^\text{Fix all other token shapes} \\
    &+ w_1 \overbrace{  \frac{1}{|C|}\sum_{c \in C} \| \texttt{appearance}_{t,\text{orig}}(c) - \texttt{appearance}_{t}(c) \|_1 }^\text{Fix all appearances} \\
    &+ w_2 \overbrace { \frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|} \| \texttt{size}_{i,t,\text{orig}}(n_k) - \texttt{size}_{i,t}(n_k) \|_1 }^\text{Fix $n_k$'s size} \\
    &+ w_3 \underbrace { \frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|} \| \texttt{target\_centroid} - \texttt{centroid}_{i,t}(n_k) \|_1 }_\text{Change $n_k$'s position}
\end{aligned}
\label{eqn:moveobj2}
\end{equation}
Where $\texttt{target\_centroid}$ can be computed as a shfited version of the timestep-and-attention-specific $\texttt{centroid}_\text{orig}$ if desired, or selected to be an absolute value on the canvas (repeated across all timesteps).
We generally use weights $w_0 \in [0.5, 2],w_1 \in [0.03,0.3],  w_2 \in [0.5, 2], w_3 \in [1, 3]$.

We can also choose to guide only nouns, changing the first two summands to $\sum_{n \neq n_k}$ from $\sum_{c \neq n_k}$.

\paragraph{Resizing objects.}

We can follow Eqn.~\ref{eqn:moveobj} to resize objects as well, by setting $\mathcal{T}$ to upsample or downsample the original mask. We can similarly use Eqn.~\ref{eqn:moveobj2}, omitting the final term and setting the target \texttt{size} to a desired value, either computed as a function of $\texttt{size}_\text{orig}(n_k)$ or provided as an absolute proportion of pixels on the canvas that the object should cover. We use the same weight range for all weights except we set $w_2 \in [1, 3], w_3=0$ for Eqn.~\ref{eqn:moveobj2}.
\paragraph{Sampling new appearances.}
Generating new appearances for the same layout only requires holding the layout fixed while letting the rest vary implicitly.
\begin{equation}
\begin{aligned}
    g &= w_0 \overbrace{  \frac{1}{|C|} \sum_{c \in C}\frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|}   \| \texttt{shape}_{i,t,\text{orig}}(c) - \texttt{shape}_{i,t}(c) \|_1 }^\text{Fix all token shapes}
\end{aligned}
\label{eqn:newapps}
\end{equation}
Where we set $w_0 \in [0.1, 1]$. Generally, higher values lead to extremely precise layout preservation at the expense of diversity in appearance.

\paragraph{Sampling new layouts.}
Just as we can find new appearances for a scene of a given layout, we can perform the opposite operation, finding new layouts for scenes where objects have a given appearance:
\begin{equation}
\begin{aligned}
    g &= w_0 \overbrace{  \frac{1}{|O|} \sum_{o \in O} \| \texttt{appearance}_{t,\text{orig}}(n) - \texttt{appearance}_{t}(n) \|_1 }^\text{Fix all appearances} 
\end{aligned}
\label{eqn:newlays}
\end{equation}
We almost always use $w_0 \in [0.05,0.25]$.
\paragraph{Collaging objects in-place.}
Say we have $J$ images, where we are interested in transferring the appearance of a single object $n_{k_j}$ from each one. We can collage these objects ``in-place'', {\em i.e.} maintaining their size, shape, position, and appearance, as one might expect -- by introducing terms to satisfy all of those constraints:
\begin{equation}
    \begin{aligned}
       g &=  w_0 \overbrace{\frac{1}{J} \sum_j \frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|}  \| \texttt{shape}_{i,t,j}(n_{k_j}) -\texttt{shape}_{i,t}(n_{k_j})  \|_1}^\text{Copy each object's shape, position, and size} \\
       &+ w_1 \underbrace{\frac{1}{J} \sum_j  \| \texttt{appearance}_{t,j}(n_{k_j}) - \texttt{appearance}_{t}(n_{k_j}) \|_1 }_\text{Copy each object's appearance}
    \end{aligned}
\end{equation}


\begin{figure}
    \input{figures/supp/newapps}
    \caption{\textbf{Creating new appearances for scenes.} Random, non-cherry-picked results sampling different ``styles'' of appearances given the same layout, using Eqn.~\ref{eqn:newapps}. We use $w_0=0.7$, $0.3$, and $0.3$ respectively for each result, to preserve greater structure in the background of the first picture.}
    \label{fig:newappsupp}
    \vspace{-1em}
\end{figure}
This can be easily generalized to more than one object per image (adding another sum across all objects) or to the case where prompts vary between images (mapping from $k_j$ to the corresponding indices in the new image). We set $w_0 \in [0.5,1], w_1 \in [0.05, 0.3]$.
\paragraph{Transferring object appearances to new layouts.}

\begin{figure}
    \input{figures/supp/newlayouts}
    \caption{\textbf{Creating new layouts for scenes.} Random, non-cherry-picked results sampling new layouts for the same scenes, using Eqn.~\ref{eqn:newlays}. We use $w_0=0.07$, $0.07$, and $0.2$ respectively.}
    \label{fig:newlaysupp}
    \vspace{-1em}
\end{figure}

Nothing requires the indices (or in fact, the objects those indices refer to) to be the same in the image being generated and the original image being used as a source, as long as there is a mapping specified between the indices in the old and new images which should correspond. Call this mapping $m$. We can then take the appearance of an object $n_k$ in a source image and transfer it to an image with any new prompt as follows:
\begin{equation}
    g = w_0 \overbrace{\| \texttt{appearance}_{t,\text{orig}}(n_{k}) - \texttt{appearance}_{t}\left(m(n_{k})\right) \|_1}^\text{Copy object appearance}
    \label{eqn:objappxfer}
\end{equation}
With weights $w_0 \in [0.01, 0.1]$.
\paragraph{Merging layout and appearance.} Combining the layout of image $A$ with the appearance of objects in image $B$ is straightforward (we set $w_0 \in [1,2]$ and $w_1 \in [0.1,0.3]$):
\begin{equation}
\begin{aligned}
    g &=  w_0 \overbrace{  \frac{1}{|C|} \sum_{c \in C}\frac{1}{|\mathcal{A}|} \sum_{i=0}^{|\mathcal{A}|}   \| \texttt{shape}_{i,t,A}(c) - \texttt{shape}_{i,t}(c) \|_1 }^\text{Copy token shapes from A} \\
    &+ w_1 \overbrace{  \frac{1}{|C|} \sum_{c \in C} \| \texttt{appearance}_{t,B}(c) - \texttt{appearance}_{t}(c) \|_1 }^\text{Copy token appearance from B} 
\end{aligned}
\end{equation}
\paragraph{Editing with real images.} Importantly, our method is not limited to editing generated images to whose internals it has access by definition. We find that we can also meaningfully guide generation using the attention and activations extracted from a set of forward-process denoisings of a real image (given a caption) to ``approximate'' the reverse process, despite any mismatch in distributions one might imagine. Concretely, we generate $T$ corrupted versions of a real image $x$, $\{ \alpha_t x + \sigma_t \epsilon_t \}_1^T$, where $\epsilon_t \sim \mathcal{N}(0,1)$. We then extract the attention $\mathcal{A}_t$ and activations $\Psi_t$ from the denoising network at each of these timesteps in parallel and concatenate them into a length-$T$ sequence. We treat this sequence identically to a sequence of $T$ internals given by subsequent sampling steps, and can thus transfer the appearance of objects from real images, output images that look like real images with moved or resized objects, and so on.

In Figure~\reff{fig:appearance_transfer}{6} in the main paper, the prompts we use to transfer appearance are ``A photo of a Chow Chow...'' and ``A DSLR photo of a teapot...''. While our method works on less specific descriptions as well, it is not as reliable when object appearance is more out-of-distribution. For context, we show unguided samples under the prompts from Figure~\reff{fig:appearance_transfer}{6} in the main paper in Figure~\ref{fig:realimgsamepromptsupp}, which still deviate significantly from the desired appearance, showing the efficacy of our approach.%

\paragraph{Weight selection heuristics.} We find weights that work well to remain more or less consistent across different images given an edit, but ideal weights do vary somewhat between different combinations of terms. Our heuristics for weight selection per term are: the more weights there are, the higher per-term weights can be without causing artifacts (and indeed, need to be, to provide ample contribution to the final result); \texttt{appearance} terms should have weights 1 or 2 orders magnitude lower than layout terms; layout summary statistics (\texttt{centroid} and \texttt{size}) should have slightly lower terms than terms on the per-pixel \texttt{shape}; total weight of terms should not add up to more than $\sim 5$ to avoid artifacts.
\subsection{Additional results}
We show non-cherry-picked results for the edits we show in the main paper. Our general protocol consists of selecting an interesting prompt manually, verifying that our model creates compelling samples aligning with this prompt without self-guidance, beginning with the typical weights we use for an edit, and trying around 3-5 other weight configurations to find the one that works best for the prompt -- in most cases, this is the starting set of weights. Then, we use the first 8 images we generate, without further filtering. We generate all results with different seeds to showcase the strength of guidance even without shared DDPM noise. We show more results for moving (Fig.~\ref{fig:moveobjsupp}) and resizing (Fig.~\ref{fig:resizeobjsupp}) objects, sampling new appearances for given layouts (Fig.~\ref{fig:newappsupp}) as well as new layouts for a given set of objects (Fig.~\ref{fig:newlaysupp}), transferring the appearance of real objects into new contexts (Fig.~\ref{fig:realimgappsupp}),



\begin{figure}
    \input{figures/supp/realimgapp}
    \caption{\textbf{Appearance transfer from real images.} Random, non-cherry-picked results sampling new images with a given object's appearance specified by real images, as in Eqn.~\ref{eqn:objappxfer}. We use $w_0=0.15$.}
    \label{fig:realimgappsupp}
    \vspace{-0.5em}
\end{figure}

\begin{figure}
    \input{figures/supp/realimgsameprompt}
    \caption{\textbf{Ablating appearance transfer from real images.} To verify the efficacy of our approach, we compare our results from Figure~\reff{fig:appearance_transfer}{6} in the paper to random samples from the same prompt without appearance transfer. We can see that appearance of objects varies significantly without self-guidance.}
    \label{fig:realimgsamepromptsupp}
    \vspace{-1em}
\end{figure}


